Band Relevance Factor (BRF): a novel automatic frequency band selection method based on vibration analysis for rotating machinery

The monitoring of rotating machinery has now become a fundamental activity in the industry, given the high criticality in production processes. Extracting useful information from relevant signals is a key factor for effective monitoring: studies in the areas of Informative Frequency Band selection (IFB) and Feature Extraction/Selection have demonstrated to be effective approaches. However, in general, typical methods in such areas focuses on identifying bands where impulsive excitations are present or on analyzing the relevance of the features after its signal extraction: both approaches lack in terms of procedure automation and efficiency. Typically, the approaches presented in the literature fail to identify frequencies relevant for the vibration analysis of a rotating machinery; moreover, with such approaches features can be extracted from irrelevant bands, leading to additional complexity in the analysis. To overcome such problems, the present study proposes a new approach called Band Relevance Factor (BRF). BRF aims to perform an automatic selection of all relevant frequency bands for a vibration analysis of a rotating machine based on spectral entropy. The results are presented through a relevance ranking and can be visually analyzed through a heatmap. The effectiveness of the approach is validated in a synthetically created dataset and two real dataset, showing that the BRF is able to identify the bands that present relevant information for the analysis of rotating machinery.

==> mybib_referencias.tex <==
@article{QIU20061066,
title = "Wavelet filter-based weak signature detection method and its application on rolling element bearing prognostics",
journal = "Journal of Sound and Vibration",
author = "Hai Qiu and Jay Lee and Jing Lin and Gang Yu",
volume = "289",
number = "4",
pages = "1066 - 1090",
year = "2006"}


@article{IMS_dataset,
  title={Bearing dataset},
  author={Lee, J and Qiu, H and Yu, G and Lin, Ja},
  journal={IMS, University of Cincinnati, NASA Ames Prognostics Data Repository, Rexnord Technical Services, Moffett Field, CA, Available online: https://ti.arc.nasa.gov/tech/dash/pcoe/prognostic-data-repository/#bearing (accessed on 14 November 2021)},
  year={2007}
}

Lee, J.; Qiu, H.; Yu, G.; Lin, J. Rexnord Technical Services, IMS, University of Cincinnati. Bearing Data Set, NASA Ames Prognostics Data Repository. NASA Ames Research Center, Moffett Field, CA. Available online: https://ti.arc.nasa.gov/tech/dash/pcoe/prognostic-data-repository/#bearing (accessed on 14 November 2021).

@article{brito2021explainable,
      title={An Explainable Artificial Intelligence Approach for Unsupervised Fault Detection and Diagnosis in Rotating Machinery}, 
      author={Lucas Costa Brito and Gian Antonio Susto and Jorge Nei Brito and Marcus Antonio Viana Duarte},
      journal={Mech. Syst. Signal Process},
      volume = {163},
      pages = {108105},
      year = {2022},
}  

@article{Canedo,
title = " A review of feature selection methods on synthetic data",
author = "Bolón Canedo, V. and Sánchez Maroño, N. and Alonso Betanzos, A",
journal = {Knowl Inf Syst},
volume = "34",
pages = "483 - 519",
year = "2013",
}

@article{ZHANG20112941,
title = "Feature selection for high-dimensional machinery fault diagnosis data using multiple models and Radial Basis Function networks",
journal = "Neurocomputing",
volume = "74",
number = "17",
pages = "2941 - 2952",
year = "2011",
author = "Kui Zhang and Yuhua Li and Philip Scarf and Andrew Ball"}

@article{ZHANG20182426,
title = "A two-stage feature selection and intelligent fault diagnosis method for rotating machinery using hybrid filter and wrapper method",
journal = "Neurocomputing",
volume = "275",
year = "2018",
author = "Xiaolong Zhang and Qing Zhang and Miao Chen and Yuantao Sun and Xianrong Qin and Heng Li"}
%pages = "2426 - 2439",


@article{LEI20091535,
title = "Gear crack level identification based on weighted K nearest neighbor classification algorithm",
journal = "Mech. Syst. Signal Process",
volume = "23",
number = "5",
pages = "1535 - 1547",
year = "2009",
issn = "0888-3270",
author = "Yaguo Lei and Ming J. Zuo"
}

@article{LI2017295,
title = "A fault diagnosis scheme for planetary gearboxes using modified multi-scale symbolic dynamic entropy and mRMR feature selection",
journal = "Mechanical Systems and Signal Processing",
volume = "91",
pages = "295 - 312",
year = "2017",
issn = "0888-3270",
author = "Yongbo Li and Yuantao Yang and Guoyan Li and Minqiang Xu and Wenhu Huang"}

@article{SINGH2019524,
title = "Faulty bearing detection, classification and location in a three-phase induction motor based on Stockwell transform and support vector machine",
journal = "Measurement",
volume = "131",
pages = "524 - 533",
year = "2019",
issn = "0263-2241",
author = "Megha Singh and Abdul Gafoor Shaik"}

@article{SMITH2015100,
title = "Rolling element bearing diagnostics using the Case Western Reserve University data: A benchmark study",
journal = "Mechanical Systems and Signal Processing",
volume = "64-65",
pages = "100 - 131",
year = "2015",
issn = "0888-3270",
author = "Wade A. Smith and Robert B. Randall"}

@article{xjtu_sy,
  author = {B. Wang and Y. Lei and N. Li and N. Li},
  title = {A Hybrid Prognostics Approach for Estimating Remaining Useful Life of Rolling Element Bearings},
  journal = {IEEE Transactions on Reliability},
  volume = {69},
  year = {2020},
  pages = {401-412}
}

@article{LEI2020106587,
author = "Yaguo Lei and Bin Yang and Xinwei Jiang and Feng Jia and Naipeng Li and Asoke K. Nandi",
title = "Applications of machine learning to machine fault diagnosis: A review and roadmap",
journal = "Mechanical Systems and Signal Processing",
volume = "138",
pages = "106587",
year = "2020",
issn = "0888-3270"}

@article{LEI20072280,
author = "Yaguo Lei and Zhengjia He and Yanyang Zi and Qiao Hu",
title = "Fault diagnosis of rotating machinery based on multiple ANFIS combination with GAs",
journal = "Mechanical Systems and Signal Processing",
volume = "21",
number = "5",
pages = "2280 - 2294",
year = "2007",
issn = "0888-3270"}

@article{LEI20101419,
author = "Yaguo Lei and Ming J. Zuo and Zhengjia He and Yanyang Zi",
title = "A multidimensional hybrid intelligent method for gear fault diagnosis",
journal = "Expert Systems with Applications",
volume = "37",
number = "2",
pages = "1419 - 1430",
year = "2010",
issn = "0957-4174"}

@book{Goodfellow-et-al-2016,
    title={Deep Learning},
    author={Ian Goodfellow and Yoshua Bengio and Aaron Courville},
    publisher={MIT Press},
    note={\url{http://www.deeplearningbook.org}},
    year={2016}
}

@book{dimen_red,
    title={Open Problems in Spectral Dimensionality Reduction},
    author={H. Strange and R. Zwiggelaar},
    publisher={Briefs in Computer Science},
    year={2014}
}

@book{pca,
    title={Principal Component Analysis},
    author={I.T. Jolliffe},
    publisher={New York: Springer-Verlag},
    year={1986}
}

@article{isomap,
  author = {J.B. Tenenbaum and V. de Silva and J.C. Langford},
  title = {A global geometric framework for nonlinear dimensionality reduction},
  journal = {Science},
  volume = {290},
  year = {2000},
  pages = {2319–2322}
}

@article{tsne,
  author = {L. VanDerMaaten and G. Hinton},
  title = {Visualizing Data Using t-SNE},
  journal = {Jour. of Machine Learning Research},
  volume = {9},
  year = {2008},
}

@article{ica,
  author = {C. Jutten and J. Hérault},
  title = {Blind separation of sources, part I: an adaptive algorithm based on neuromimetic architecture},
  journal = {Signal Process},
  volume = {24},
  year = {1991}
}

@article{ica_2,
  author = {A. Hyvärinen and E. Oja},
  title = {Independent component analysis: algorithms and applications},
  journal = {Neural Netw.},
  volume = {13(4–5)},
  year = {2000},
  pages = {411–430}
}

@article{micro,
  author = {Milla Caroline Gomes and Lucas Costa Brito and Márcio Bacci da Silva and Marcus Antônio Viana Duarte},
  title = {Tool wear monitoring in micromilling using Support Vector Machine with vibration and sound sensors},
  journal = {Precision Engineering},
  volume = {67},
  year = {2021},
  pages = {137-151}
}

@article{mestrado,
  author = {Lucas Costa Brito and M.B. da Silva and M.A.V Duarte},
  title = {Identification of cutting tool wear condition in turning using self-organizing map trained with imbalanced data},
  journal = {J Intell Manuf},
  volume = {32},
  year = {2021},
  pages = {127–140}
}

@article{LIU201833,
author = "Ruonan Liu and Boyuan Yang and Enrico Zio and Xuefeng Chen",
title = "Artificial intelligence for fault diagnosis of rotating machinery: A review",
journal = "Mechanical Systems and Signal Processing",
volume = "108",
pages = "33 - 47",
year = "2018"}

@article{Kumar,
author = {Prashant Kumar and Ananda Shankar Hati},
title = {Review on Machine Learning Algorithm Based Fault Detection in Induction Motors},
journal = {Arch Computat Methods Eng},
volume = {},
pages = {1-12},
year = {2020},
}

@article{STETCO2019620,
author = "Adrian Stetco and Fateme Dinmohammadi and Xingyu Zhao and Valentin Robu and David Flynn and Mike Barnes and John Keane and Goran Nenadic",
title = "Machine learning methods for wind turbine condition monitoring: A review",
journal = "Renewable Energy",
volume = "133",
pages = "620 - 635",
year = "2019",
}

@article{barbariol2020self,
  title={Self-Diagnosis of Multiphase Flow Meters through Machine Learning-Based Anomaly Detection},
  author={Barbariol, Tommaso and Feltresi, Enrico and Susto, Gian Antonio},
  journal={Energies},
  volume={13},
  number={12},
  pages={3136},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{rai2020fraud,
  title={Fraud Detection in Credit Card Data using Unsupervised Machine Learning Based Scheme},
  author={Rai, Arun Kumar and Dwivedi, Rajendra Kumar},
  booktitle={2020 International Conference on Electronics and Sustainable Communication Systems (ICESC)},
  pages={421-426},
  year={2020},
  organization={IEEE}
}

@article{zhao2019pyod,
  author  = {Zhao, Yue and Nasrullah, Zain and Li, Zheng},
  title   = {PyOD: A Python Toolbox for Scalable Outlier Detection},
  journal = {Journal of Machine Learning Research},
  year    = {2019},
  volume  = {20},
  number  = {96},
  pages   = {1-7}
  }

@article{if_1, 
  author = {Fei Tony Liu and Kai Ming Ting and Zhi-Hua Zhou},
  title = {Isolation forest},
  journal = {ICDM},
  volume = {},
  year = {2008},
  pages = {413–422}
}

@article{if_2, 
  author = {Fei Tony Liu and Kai Ming Ting and Zhi-Hua Zhou},
  title = {Isolation-Based Anomaly Detection},
  journal = {ACM Trans. Knowl. Discov. Data},
  volume = {6},
  year = {2012},
  pages = {1-39}
}

@misc{zocco2021greedy,
      title={Greedy Search Algorithms for Unsupervised Variable Selection: A Comparative Study}, 
      author={Federico Zocco and Marco Maggipinto and Gian Antonio Susto and Seán McLoone},
      year={2021},
      eprint={2103.02687},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{lei2013,
  author = {Y. Lei and J. Lin and Z. He and M. J. Zuo},
  title = {A review on empirical mode decomposition in fault diagnosis of rotating machinery},
  journal = {Mech. Syst. Signal Process},
  volume = {35},
  year = {2013},
  pages = {108–126}
}

@article{pdm,
  author = {Bousdekis, Alexandros and Magoutas, Babis and Apostolou, Dimitris and Mentzas, Gregoris},
  title = {Review, analysis and synthesis of prognostic-based decision support methods for condition based maintenance},
  journal = {Journal of Intelligent Manufact.},
  volume = {29},
  year = {2018},
  pages = {1303–1316}
}

@article{feature01,
  author={L. {Ciabattoni} and F. {Ferracuti} and A. {Freddi} and A. {Monteriù}},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Statistical Spectral Analysis for Fault Diagnosis of Rotating Machines}, 
  year={2018},
  volume={65},
  number={5},
  pages={4301-4310}}
  
@article{feature04,
    author = {Wei, Y. and Li, Y and Xu, M. and Huang, W.},
    title = {A Review of Early Fault Diagnosis Approaches and Their Applications in Rotating Machinery},
    journal = {Entropy},
    year = {2019},
    volume = {21},
    number = {4},
    pages = {409}}
    
@book{hawkinsbook,
  title={Identification of outliers},
  author={D Hawkins},
  year={1980)},
  publisher={Chapman and Hall}
}    

@article{benchmark_bearing,
    author = {Diallo, M.S. and Mokeddem, S.A. and Braud, A. and Frey, G. and Lachiche, N.},
    title = {Identifying Benchmarks for Failure Prediction in Industry 4.0},
    journal = {Informatics},
    year = {2021},
    volume = {8},
    number = {8},
    pages = {68}}
